Living IoT: A Flying Wireless Platform on Live Insects

Sensor networks with devices capable of moving could enable applications ranging from precision irrigation to environmental sensing. Using mechanical drones to move sensors, however, severely limits operation time since flight time is limited by the energy density of current battery technology. We explore an alternative, biology-based solution: integrate sensing, computing and communication functionalities onto live flying insects to create a mobile IoT platform. Such an approach takes advantage of these tiny, highly efficient biological insects which are ubiquitous in many outdoor ecosystems, to essentially provide mobility for free. Doing so however requires addressing key technical challenges of power, size, weight and self-localization in order for the insects to perform location-dependent sensing operations as they carry our IoT payload through the environment. We develop and deploy our platform on bumblebees which includes backscatter communication, low-power self-localization hardware, sensors, and a power source. We show that our platform is capable of sensing, backscattering data at 1 kbps when the insects are back at the hive, and localizing itself up to distances of 80 m from the access points, all within a total weight budget of 102 mg.

==> accel.tex <==
\subsubsection{Improving localization and achieving 3D tracking}\label{subsubsec:accel} Insects exhibit characteristic motion during flight that we can exploit to improve localization. Bees, which have been particularly well studied, flap their wings approximately 200 times per second. Moreover, bumblebees typically fly along straight line paths with average speeds of 3~m/s~\cite{beespeed} and hover around colorful objects such as flowers  while foraging. By taking advantage of these foraging and motion patterns, we can improve our localization accuracy.

To enable this, we attach an $1.1 \times 1.3$~mm, low power 3-axis accelerometer to the insect~\cite{mcube}. The accelerometer provides the acceleration data along the 3 axes. We combine this data with the RF 2D location estimate as follows.
\squishlist
\item {\it Estimating Z coordinate.} Since bees typically fly along straight lines, the acceleration along the z axis is minimal and occurs only when the insects hover near the flowers or face any obstacles. We take advantage of this behavior to localize the insect in a 3-D space. Given the height of the hive as the initial Z coordinate, we use the accelerometer data along the z axis to update the location of the insect in the 3D space. We note that since the motion along the z axis is minimum, confined to a limited range of values and not continuous, the error contribution to 3D localization due to accelerometer errors is small.

\item {\it Improving localization.} Using the acceleration measurement along the x and y axes, we can compute the speed and the distance traveled by the insect over a short duration. We can combine this estimate with the RF location estimate to improve the localization accuracy. Specifically, we first compute an estimate of the distance from the RF signal. We then combine the displacement estimated by the accelerometer with the RF estimate where the weight for the accelerometer is proportional to the distance from the AP. Specifically, at longer distances, the accelerometer data is given more weight while the RF data is given a larger weight at closer distances.  As we do not rely only on the accelerometer data but instead combine it with RF data, we minimize the error accumulation of the accelerometer data over time.
\squishend
% do we need to add this ?
%\vskip 0.05in\noindent{\bf Hovering motion.} Insects hover around a flower in a specific manner. While hovering, the location of the insect does not change significantly. If we can identify the hovering pattern using the accelerometer data, we need not recompute the location estimate in that duration, thus saving power on the insect. 

